Development of Cryogenic Scintillation Detectors for the Search of New Physics

CryoCsI, the proposed prototype, is a cryogenic undoped CsI scintillating detector, which has a much lower energy threshold potentially down to 0.5 keV$_{nr}$ compared to the doped CsI. This enhanced sensitivity of CryoCsI allows for the observation of more Coherent elastic neutrino-nucleus scattering events. Precise measurements of CEvNS can not only validate the predictions of the Standard Model but also explore new physics. In conjunction with other COHERENT detectors, CryoCsI has the potential to achieve world-leading sensitivities in a broad range of physics topics within and beyond the SM. The sensitivities of CryoCsI to hidden-sector dark matter, non-standard neutrino interactions, and neutron radius are explored. This thesis delves into the construction of CryoCsI and efforts to enhance its light yield from 20 to $50 \pm 2$ photoelectrons per keV electron-equivalent (keV$_{ee}$). It will address challenges with cryogenic SiPMs, including inferior energy resolution, optical cross-talk, and potential limitations on detecting rare events. Understanding the light yield of scintillating detectors for nuclear recoils is crucial, as explored through alpha-particle and neutron quenching factor measurements. A QF of approximately 15\% was measured using a neutron beam at the Triangle Universities Nuclear Lab. Proposed solutions to challenges like the overshoot effect observed in PMTs will be discussed. Additionally, the thesis will explore design considerations for minimizing background noise and optimizing the CsI crystal's shape through optical simulations.

==> Section2/CEvNS_experiments.tex <==
\section{CEvNS experiments}
\label{s:map}
\hspace{0.5cm} CEvNS is rapidly captivating the scientific community and evolving into a truly global endeavor. As illustrated in Table \ref{t:map}, a summary of CEvNS experiments reveals their widespread deployment across the globe. Neutrino sources for CEvNS detection fall into two categories: accelerator-based sources (see Section \ref{s:sns}) and nuclear reactors (via beta decay), chosen for their high flux and suitable energy range. To detect the subtle energy deposits from CEvNS events, three different types of signals have been utilized, leveraging phonon signatures (lattice vibrations), light signatures (photon scintillation), and charge signatures (ionization). Further details regarding neutrino sources and detector technologies for CEvNS detection will be introduced in subsequent sections.
\begin{table}[htbp]
\captionof{table}{Summary of CEvNS experiments worldwide, including details on detectors, locations, neutrino sources, neutrino fluxes, and overburden~\cite{CEvNSmapTable, CEvNSmapTable1,CEvNSmapTableBULLKID, CEvNSmapTableCCM, CEvNSmapTableESS, CEvNSmapTableNEWSG, CEvNSmapTableVio, CEvNSmapTableSBC, su_csi}. }\label{t:map}
\renewcommand{\arraystretch}{1.5}
\centering
\begin{tabular}{|m{2.3cm}|m{3cm}|m{1.6cm}|m{1.5cm}|m{2.3cm}|m{2.3cm}|}
    \hline
    \textbf{Experiment} & \textbf{Detectors} & \textbf{Location} & \textbf{Source} & \textbf{$\nu$ Flux} & \textbf{Overburden} \\ \hline
    COHERENT & CsI, LAr, Ge, NaI & USA & $\pi$DAR & $4.7\times10^{7}$ & 8 \\ \hline
    CCM & LAr & USA & $\pi$DAR & $4.74\times10^{5}$ & ? \\ \hline
    Ref.~\cite{CCEvNS, win23} & CsI,  CsI(Na), CsI, Ge, LAr, LXe, PbWO$_4$ & China & $\pi$DAR Reactor & \hspace*{-2.5mm}\begin{tabular}{l}$2\times10^{7}$ \\$2.5-6\times10^{12}$\end{tabular} & \hspace*{-2.5mm}\begin{tabular}{l}? \\ $\sim$30\end{tabular} \\ \hline
    ESS & CsI, Si, Ge, Xe & Sweden & $\pi$DAR & $4.3\times10^{8}$ & ? \\ \hline
    BULLKID & Si/Ge & Italy & Reactor & ? & ? \\ \hline
    CONNIE & Skipper CCDs & Brazil & Reactor & $6.8\times10^{12}$ & 0 \\ \hline
    CONUS & HPGe & Germany & Reactor & $2.4\times10^{13}$ & 10-45 \\ \hline
    NEWS-G & LAr + 2\%CH$_4$ & Canada & Reactor & $7\times10^{11}$ & 0 \\ \hline
    MINER & cryogenic Ge/Si & USA & Reactor & $2\times10^{12}$ & $\sim$5 \\ \hline
    NEON & NaI(Tl) & Korea & Reactor & $7.1\times10^{12}$ & $\sim$20 \\ \hline
    NUCLEUS & cryogenic CaWO$_4$/Al$_2$O$_3$ & Europe & Reactor & $2\times10^{12}$ & $\sim$3\\ \hline
    $\nu$GEN & Ge PPC & Russia & Reactor & $>5\times10^{13}$ & $\sim$50 \\ \hline
    $\nu$ioleta & Skipper CCDs & Argentina & Reactor & ? & ? \\ \hline
    RED-100 & LXe dual phase & Russia & Reactor & $1.7\times10^{13}$ & $>50$ \\ \hline
    Ricochet & cryogenic Ge, Zn, Al, Sn & France & Reactor & $2\times10^{12}$ & $\sim$15 \\ \hline
    TEXONO & p-PCGe & Taiwan & Reactor & $6.4\times10^{12}$ & $\sim$30 \\ \hline
    Dresden II & PCGe & USA & Reactor & $8.1\times10^{13}$ & $\sim$27 \\ \hline
    SBC & Scintillation Bubble Chamble & USA & Reactor & ? & ? \\ \hline
    \end{tabular}\\
    ? indicates not found. The unit of neutrino flux is $\nu$/cm2/s. The unit of overburden is meters water equivalent (m w.e.). 
\end{table}

\subsection{Neutrino sources}
\hspace{0.5cm} Various neutrino sources at Earth span different energy regions, as illustrated in Fig.~\ref{f:vSources}. Reactors serve as high-flux generators of MeV-scale neutrinos, rendering them ideal for CEvNS studies. In the figure, the reactor flux is derived from a 140~MW thermal power and a detector situated 81~m away. Notably, CEvNS experiments typically employ reactors with significantly higher power and neutrino flux, as detailed in Table~\ref{t:map}. In contrast, other sources either yield low-flux neutrinos or necessitate exceedingly sensitive detectors due to the exceptionally low-energy neutrinos. Note that neutrinos generated from the SNS are not discussed here. In the figure, BBN stands for the Big Bang nucleosynthesis, CNB is the cosmic neutrino background, and DSNB represents the diffuse supernova neutrino background. Each of these sources presents distinct challenges and opportunities for researchers exploring the intricacies of neutrino interactions across the energy spectrum.
\begin{figure}[ht!]\centering
    \includegraphics[width=0.9\linewidth]{Section2/vSources.png}
    \caption{Grand Unified Neutrino Spectrum on Earth from Ref.~\cite{vSources}, integrated over directions and summed over flavors. Therefore, flavor conversion between source and detector does not affect this plot. Solid lines are for neutrinos, dashed or dotted lines for antineutrinos, superimposed dashed and solid lines for sources of both neutrinos and antineutrinos. }
    \label{f:vSources}
\end{figure}

As shown in Fig.~\ref{f:SorR}, the pion decay-at-rest ($\pi$DAR, SNS) source produces 30~MeV neutrinos, maintaining an energy level that is not excessively high to compromise coherence while also allowing for a relatively lower detection threshold. Additionally, the SNS beam exhibits high background rejection. Reactors, on the other hand, generate a higher flux of neutrinos within a good energy region to maintain coherence. However, careful attention must be paid to background considerations in reactor-based experiments. Thus far, CEvNS has only been observed from the SNS source. Fig.~\ref{f:sns} shows the current and future $\pi$DAR sources, with the SNS standing out for its combination of high flux and a substantial factor for background rejection.
\begin{figure}[ht!]\centering
    \includegraphics[width=\linewidth]{Section2/SorR.png}
    \caption{Neutrino flux from various sources across a range of neutrino energies~\cite{CEvNSmapTable1}. Listed reactor neutrinos are particularly favorable for CEvNS scatterings, exhibiting higher flux compared to the SNS.}
    \label{f:SorR}
\end{figure}

\begin{figure}[ht!]
    \includegraphics[width=\linewidth]{Section2/SNS.png}\centering
    \caption{Figures of merit for stopped-pion neutrino sources worldwide (past, current and future)~\cite{snowmassCO22}.  The x-axis shows the total (all-flavor) neutrino flux, which depends on the beam power and proton energy, as well as details of the target geometry.  The uncertainty is shown as the range of fluxes.  The diamonds show flux estimates based on Geant4 QGSP\_BERT; the circles indicate the relevant collaboration's chosen baseline flux estimate. The y-axis shows the inverse square root of the duty factor, a measure of impact of background rejection due to beam pulsing, where duty factor is determined from the maximum of the muon decay lifetime, 2.2~$\mu$s, and the beam pulse window (1~$\mu$s).   A larger value corresponds to improved steady-state background rejection.    The diagonal lines represent contours of equal flux over inverse square root of the duty factor.} \label{f:sns}
  \end{figure}

\subsection{Technologies to detect CEvNS}
\hspace{0.5cm} There are three distinct signals to measure the recoiling particles: ionization/charge, scintillation/light and phonon/heat~\cite{detetcors}. Consequently, three types of detectors were utilized for CEvNS detection. The integration of these channels facilitated background discrimination between nuclear recoil signals and electron recoil signals. For instance, scintillating cryogenic calorimeters could capture phonon and light signals~\cite{cresst19} and cryogenic calorimeters with charge readout could record both phonon and charge signals~\cite{EDELWEISS10}. The liquid noble dual-phase Time Projection Chamber (TPC) is a specialized design that employs an electric field in liquid noble gas and can read out scintillation light from both excitation and ionization~\cite{ds20k}.

Ionization detectors, such as Ge, necessitate operation at low temperatures (e.g., liquid nitrogen temperature) to suppress the thermal motion of electrons. An electric field is applied to separate charges, drifting the generated electron-hole pairs in semiconductors or electron-ion pairs in gases. Compared to scintillation detectors, ionization detectors with smaller band gaps exhibit superior energy resolution. Gas detectors, in particular, have the additional capability of providing directionality.

Scintillation detectors can be categorized into organic scintillators and inorganic scintillators. Organic scintillators include materials like plastic and liquid scintillators. Inorganic scintillators encompass CsI, CsI(Na), NaI, NaI(Tl), etc., along with liquid noble gases such as LAr and LXe. LAr and organic scintillators are capable of being constructed on large mass scales reaching ton scales at a managble price. LAr's pulse shape discrimination feature allows the differentiation between electron and nuclear recoils. However, scintillators exhibit relatively poor energy resolution compared to ionization or phonon detectors. Normally, PMTs, avalanche photodiodes (APDs) and silicon photomultipliers (SiPMs) are used to read out the light signals emitted from scintillators.

Phonon detectors (e.g., Ge, Si, Zn, Al, Sn, PbWO$_4$, CaWO$_4$, Al$_2$O$_3$, etc.) typically function as absorbers, cooled down to millikelvin (mK) temperatures in a thermal bath. The resulting phonon interactions are read out using specialized thermometers like transition edge sensors (TES), neutron transmutation doped (NTD) thermometers, and kinetic inductance detectors (KIDs), etc. These thermometers effectively transform the heat signal into a readable electrical signal. Phonon detectors are capable of reaching eV energy thresholds due to minimized thermal noise. These bolometers offer versatility in the choice of target materials; however, the mass scale is limited to below kg.


